Learning cross-layer dependence structure in multilayer networks

We propose a novel class of separable multilayer network models to capture cross-layer dependencies in multilayer networks, enabling the analysis of how interactions in one or more layers may influence interactions in other layers. Our approach separates the network formation process from the layer formation process, and is able to extend existing single-layer network models to multilayer network models that accommodate cross-layer dependence. We establish non-asymptotic and minimax-optimal error bounds for maximum likelihood estimators and demonstrate the convergence rate in scenarios of increasing parameter dimension. Additionally, we establish non-asymptotic error bounds for multivariate normal approximations and propose a model selection method that controls the false discovery rate. Simulation studies and an application to the Lazega lawyers network show that our framework and method perform well in realistic settings.

==> abstract.tex <==
Multilayer networks are a network data structure in which elements in a population of interest have multiple modes of interaction or relation,
represented by multiple networks called layers. 
We propose a novel class of models for cross-layer dependence in multilayer networks, 
aiming to learn how interactions in one or more layers may influence interactions in other layers of the multilayer network,
by developing a class of network separable models which separate the network formation process from the multilayer formation processes. 
In our framework,
we are able to extend any existing single layer network model to a multilayer network model with cross-layer dependence. 
We establish non-asymptotic bounds on the error of estimators
and demonstrate rates of convergence for 
both maximum likelihood estimators and maximum pseudolikelihood estimators 
in scenarios of increasing parameter dimension.
We additionally establish non-asymptotic error bounds on the multivariate normal approximation and elaborate a method for model selection which controls the false discovery rate.  
We conduct simulation studies which demonstrate that our framework and method work well in realistic settings
which might be encountered in applications. 
Lastly, 
we illustrate the utility of our method through an application to the Lazega lawyers network. 


==> concentration_PL.tex <==
\begin{lemma}
\label{lem:concentration_pl}
Consider multilayer networks satisfying \eqref{general model}
which are 
defined on a set of $N \geq 3$ nodes and $K \geq 1$ layers. 
Define
$\gradPL \coloneqq - \nabla_{\nat} \, \pl(\nat; \bx, \by)$,
where $\pl(\nat; \bx, \by)$ is the log-pseudolikelihood function. 
Then,
for all $t > 0$ and $\nat \in \mbR^p$,
\beno
\mbP\left(\norm{\GradPL - \mbE \, \GradPL}_{\infty} \geq t \right)
&\leq&
2 \, \exp\left( -\dfrac{t^2}{K^2 \, (\mbE \, \norm{\bY}_1 + [D_{g}]^{+})} + \log p \right) + \dfrac{1}{\mbE \norm{\bY}_1}.  
\ee
\end{lemma}


==> proof_concentration_PL.tex <==
From \eqref{eq:log-pseudo},
the log-pseudolikelihood function is given by
\beno
\pl(\nat; \bx, \by) = \dsum_{\{i,j\} \subseteq \mN} \, \dsum_{k=1}^{K} \, 
\log \, \sepmodel(X_{i,j}^{(k)} = x_{i,j}^{(k)} \,|\, \bX_{i,j}^{(-k)} = \bx_{i,j}^{(-k)}, \bY = \by).
\ee
By Lemma \ref{lem:exp_pseudo}, 
$\sepmodel(X_{i,j}^{(k)} = x_{i,j}^{(k)} \,|\, \bX_{i,j}^{(-k)} = \bx_{i,j}^{(-k)}, \bY = \by)$ 
is an exponential family with sufficient statistic vector $s : \mbX \mapsto \mbR^p$ 
defined in Lemma \ref{lem:s_hetero} and natural parameter vector $\nat \in \mbR^p$.
Hence,  
\beno 
\nabla_{\nat} \, \pl(\nat;\bx,\by)
\=  \dsum_{\{i,j\} \subseteq \mN} \, \dsum_{k=1}^{K}  
\nabla_{\nat} \log \, \sepmodel(X_{i,j}^{(k)} = x_{i,j}^{(k)} \,|\, \bX_{i,j}^{(-k)} = \bx_{i,j}^{(-k)}, \bY = \by) \s \\
\= \dsum_{\{i,j\} \subseteq \mN} \, \dsum_{k=1}^{K} \, 
\left[ \, \bs(\bx) - \mbE_{\nat}\left[ \bs(\bX) \, | \, \bX_{i,j}^{-(k)}  = \bx_{i,j}^{(-k)}, \bY = \by \right]  \, \right],
\ee
where $\bX_{i,j}^{-(k)}$ denotes the ($K$-$1$)-dimensional 
vector of edge variables of dyad $\{i,j\}$ in $\bX_{i,j}$ which excludes the single edge variable $X_{i,j}^{(k)}$,
and by inserting the familiar form of the score equation of an exponential family 
with respect to the natural parameter vector 
\citep[e.g., Proposition 3.10, p. 32,][]{Su19}. 
Note that $\sepmodel(X_{i,j}^{(k)} = x_{i,j}^{(k)} \,|\, \bX_{i,j}^{(-k)} = \bx_{i,j}^{(-k)}, \bY = \by)$
may not belong to a minimal exponential family. 
This presents no issues as we do not require the conditional probability distributions of individual edge variables
belong to a minimal exponential family. 
Under the assumption that $(\bX, \bY)$ follow \eqref{general model}, 
the vectors $\bX_{i,j}$ ($\{i,j\} \subset \mN$) are conditionally independent given $\bY$ 
(as discussed in the proof of Lemma \ref{lem:concentration_likelihood}). 
Therefore,
the $l^{th}$ component $s_l(\bX)$ decomposes into the sum of conditionally independent Bernoulli random variables:
\beno
s_l(\bX)
\= \dsum_{\{i,j\} \subset \mN} \, s_{l,i,j}(\bX_{i,j}),
&& l \in \{1, \ldots, p\},
\ee
so that the components of $\bs(\bX)$ are sums of bounded conditionally independent random variables given $\bY$. 
Thus,
\beno
\nabla_{\nat} \, \pl(\nat;\bx,\by)
\= \dsum_{\{i,j\} \subseteq \mN} \, \dsum_{k=1}^{K} \,
\left( s_{l,i,j}(\bX_{i,j}) - E_{l,i,j}(\nat, \bx_{i,j}, \by) \right),
\ee
where
\beno
E_{l,i,j}(\nat, \bx_{i,j}, \by)
&\coloneqq& 
\mbE_{\nat}\left[s_{l,i,j}(\bX_{i,j}) \,|\, \bX_{i,j}^{(-k)} = \bx_{i,j}^{(-k)}, \bY = \by \right].
\ee
Using the form of $s_l(\bX)$ and $s_{l,i,j}(\bX_{i,j})$ outlined in Lemma \ref{lem:s_hetero},
we have $0 \le s_{l,i,j}(\bX_{i,j}) \le Y_{i,j}$ $\mbP$-almost surely,
because $s_{l,i,j}(\bX_{i,j}) \in \{0, 1\}$ and $s_{l,i,j}(\bX_{i,j}) = 0$ if $Y_{i,j} = 0$ $\mbP$-almost surely.
This also implies 
$0 \leq E_{l,i,j}(\nat, \bx_{i,j}, \by) \leq Y_{i,j}$ $\mbP$-almost surely. 
Taken together, 
\beno
0 
\,\leq\, \left| \dsum_{k=1}^{K} \,
\left( s_{l,i,j}(\bX_{i,j}) - E_{l,i,j}(\nat, \bx_{i,j}, \by) \right) \right| 
\,\leq\, \dsum_{k=1}^{K} \left| s_{l,i,j}(\bX_{i,j}) - E_{l,i,j}(\nat, \bx_{i,j}, \by) \right|  
\,\leq\, K \, Y_{i,j}, 
\ee
$\mbP$-almost surely. 
From here,
the remainder of the proof follows the proof of Lemma \ref{lem:concentration_likelihood},
with the sole exception using 
the bound $K \, Y_{i,j}$ in the application of Hoeffding's inequality. 
Reiterating the proof of Lemma \ref{lem:concentration_likelihood} with this change will yield  
\beno
\mbP\left(\norm{\GradPL - \mbE \, \GradPL}_{\infty} \geq t \right)
&\leq&
2 \, \exp\left( -\dfrac{t^2}{K^2 \, (\mbE\, \norm{\bY}_1 + [D_{g}]^{+})} + \log p \right) + \dfrac{1}{\mbE \norm{\bY}_1}.  
\ee

\qed 






==> sim_expansion.tex <==
\subsection{Simulation expansion (Under update)}

\subsubsection{Consistency of MPLE for random data-generating parameters} 
We took 250 multilayer network samples from four different model-generating parameters uniformly sampled from $[-1,1]$ at increasing network sizes from $N = 200$ to $1000$. Two density settings of the Bernoulli basis network $\bY$ are simulated: $1)$ fixed density with $\mbP(Y_{i,j} = 1) = 0.8$, and $2)$ varying densities as a function of network size $N$, i.e., $\mbP(Y_{i,j} = 1) = 20/N$. Figure \ref{consistency_dense} shows the consistency of MPLE for four different data-generating parameters in the setting of a denser basis network while Figure \ref{f_varyspars} shows the same consistency result in the setting of a sparse basis network. Another example of decay rate change due to density change will be added as well.
\begin{figure}
\includegraphics[width=\textwidth]{4theta_consistency.pdf}
	\caption{Boxplot of the relative $\ell_2$-errors of $\mple$ for 4 different data-generating parameters in the setting of a denser basis network.}
	\label{consistency_dense}
\end{figure}


\begin{figure}
\includegraphics[width=\textwidth]{mple_error_sparse.pdf}
	\caption{Boxplot of the relative $\ell_2$-errors of $\mple$ for 4 different data-generating parameters in the setting of a sparse basis network.}
	\label{f_varyspars}
\end{figure}



\hide{
The MPLE $\mple$ of the ten parameter settings are displayed in Figure \ref{f_hm1} and Figure \ref{f_hm2} with different arrangements. In Figure \ref{f_hm1}, $x$-axis is ordered by the $\ell_2$-norm of corresponding model-generating parameters while in Figure \ref{f_hm2}, the $x$-axis is ordered by the element-wise sum of each parameter, where negative or smaller values suggest a more sparse network compared to larger values. In general, networks with more edges tend to be better estimated at a finite network size. Note that, the $\ell_2$ errors in Figure \ref{f_hm1} and \ref{f_hm2} are truncated at 0.3 because some parameters do not have a converged MPLE.
\begin{figure}
\includegraphics[width=\textwidth]{boxplot-groups.png}
 
	\caption{Boxplot of the relative $\ell_2$-errors of $\mple$ ordered by the $\ell_2$-norm of the corresponding 10 parameter vectors on the $x$-axis grouped by different densities of the basis network $\bY$.}
	\label{f_hm1}
\end{figure}
\begin{figure}
\includegraphics[width=\textwidth]{boxplot-groups2.png}
 
	\caption{Boxplot of the relative $\ell_2$-errors of $\mple$ ordered by the element-wise sum of the corresponding 10 parameter vectors on the $x$-axis grouped by different densities of the basis network $\bY$.}
	\label{f_hm2}
\end{figure}
}


\subsubsection{Estimation errors and the number of layers}
\begin{figure}
\includegraphics[width=\textwidth]{heatmap_KN.png}
	\caption{Heatmap of the relative $\ell_2$-errors of $\mple$ ordered by the network size on the $x$-axis and by the number of layers on the $y$-axis.}
	\label{f_hm3}
\end{figure}
Figure \ref{f_hm3} is the heat map of the relative $\ell_2$ errors of $\mple$ at $\truth= (-3,  0.5, 0, -2, 0, -1)$, arranged by the number of layers on the $y$-axis and the network size on the $x$-axis. When the network size $N$ is small (50), more layers lead to larger estimation error. When the network size $N$ is large, the increase in the number of layers from 3 to 6 does not play a significant role in MPLE as shown in the graph.



==> simulation.tex <==
In this section, we add simulation evidence to our major contributions. Section \ref{sec:sim_con} shows the consistency results in Theorem \ref{thm1} for the pseudolikelihood estimator $\mple$. Section \ref{sec:sim_norm} shows the multivariate normality results of Theorem \ref{thm2}. In addition, we discuss several model selection procedures that control the false discovery rate (FDR) at level $\alpha$ in Section \ref{sim:sec_fdr}.


\begin{table}[t]
\begin{center}
\caption{\label{t1}Values of the model-generating parameter $\truth$ and mean of MPLE $\mple$ from 500 replications at network size 1000. Standard errors are in the parenthesis.}
\begin{tabular}{| c | c | c | c | c | c | c |} 
\hline
  & $\theta_{1}$&$\theta_{2}$&$\theta_{3}$& $\theta_{1,2}$ & $\theta_{1,3}$ & $\theta_{2,3}$ \\ 
\hline
$\truth$ & $-3$ & $-2$ & $-1$ & $.5$ & $0$ & $0$  \\
\hline
$\mple$ & $-2.999 \, (.02)$ & $-1.998 \, (.02)$ & $-.999 \, (.02)$ & $.499 \, (.02)$ & $-.001 \, (.02)$ & $-.002 \, (.02)$\\
\hline
\end{tabular}
\end{center}
\end{table}


Throughout the simulation, we sample network concordant multilayer networks $(\bX,\bY)$ with $N$ nodes and $K = 3$ layers according to model \eqref{general model}, where $\bY$ is a Bernoulli random graph with $\mbP(Y_{i,j} = 1) = g$ for all $\{i,j\} \subset \mN$, and
\beno
f(\bx, \nat) = \dprod_{i<j}^N \, \exp\left( \dsum_{k=1}^3\theta_{k}\,x_{i,j}^{(k)} + \dsum_{\substack{k < l}}^{3}\, \theta_{k,l} \, x_{i,j}^{(k)} \, x_{i,j}^{(l)} \right).
\ee
The natural parameter $\nat \in \mbR^{6}$ specifies three different layer densities through $\theta_{1},\,\theta_{2}$, and $\theta_{3}$, as well as three cross-layer interactive effects through $\theta_{1,2},\,\theta_{1,3}$, and $\theta_{2,3}$.




\section{Consistency of MPLE} 
\label{sec:sim_con}

The consistency of the maximum pseudolikelihood estimator (MPLE) is demonstrated through the decay of the relative $\ell_2$ error between the MPLE $\mple$ and the data-generating parameter $\truth$ in Figure \ref{Figure1}(a). As the network size increases from 100 to 1000, the relative $\ell_2$ error decreases to 0. For each network size, $M=500$ samples were taken. The decay rate of the relative $\ell_2$ error as the network size increases can be estimated by the slope of the OLS fitted line in the $\log$-$\log$ plot as shown in Figure \ref{Figure1}(b). The slope of the OLS line is $-1$, indicating a decay rate of order $1/N$, which follows the result in Theorem \ref{thm1}. We report the MPLE $\mple$ averaged from $M = 500$ samples with the selected model-generating parameter $\truth$ at network size 1000 in table \ref{t1}.

\begin{figure}[t]
	\includegraphics[width=\textwidth]{Box_OLS.png}
	\caption{Graph (a) on the left shows the box-plot of relative $\ell_2$ errors for $\mple$ and $\truth$ decrease to 0 as the network size increases. Graph (b) on the right shows an OLS line with slope $-1$ for the relative $\ell_2$ errors in a log-log plot, indicating an 1/N decay rate of the estimation error.}
	\label{Figure1}
\end{figure}


% \begin{figure}[htp]
% 	\includegraphics[width=\textwidth]{Boxplot_6theta_ggplot.png}
% 	\caption{The relative $\ell_2$ errors of all dimensions of $\mple$ and $\truth$ decrease to 0 as the network size increases.}
% 	\label{Figure2}
% \end{figure}



\section{Normality of MPLE} 
\label{sec:sim_norm}
As stated in Theorem \ref{thm2}, the distribution of the maximum likelihood estimator $\mle$ converges to a multivariate normal distribution as the network size increases. We show by simulation that the maximum pseudolikelihood estimators (MPLEs) are approximately multivariate normal as well. We first demonstrate through Q-Q plots in Figure \ref{Figure3} that each component of the MPLE $\mple$ follows a marginal normal distribution. 
% We constructed 95\% confidence ellipses for bivariate components of $\mple$ in figure \ref{Figure4}. The two axes in each sub-plot of figure \ref{Figure4} correspond to two different components of $\mple$. The red ellipse is the 95\% confidence ellipse generated by the mean and covariance matrix of the MPLEs in the plot under the bivariate normal assumption. All 15 bivariate confidence ellipses cover most of estimates points, suggesting probable bivariate normal distributions of $\mple$. 
The multivariate normality of $\mple$ is then tested by Zhou-Shao's multivariate normal test \citep{Zhou13}. The test failed to reject the null hypothesis that $\mple$ is multivariate normal at the significance level of 0.05, confirming that $\mple$ is multivariate normal. We additionally performed marginal tests for normality for each component. In each case, the marginal test failed to reject the null hypotheses that $\mple_i$ is marginal normal at the same significance level, for each component $i = 1,\ldots, p$, the result of which is consistent with the $Q$-$Q$ plots. 

\begin{figure}[t]
	\includegraphics[width=\textwidth]{QQplots.png}
	\caption{Q-Q plots of all dimensions of $\Tilde{\nat}$ show that the MPLEs fall on a straight line, indicating marginal normality of each dimension of $\mple$.}
	\label{Figure3}
\end{figure}


\begin{table}[t]
\begin{center}
\caption{\label{t3} Empirical FDR and power at significance level 0.05 for multiple testing of MPLE $\mple$ estimated from 500 networks of size 1000.  } 
\begin{tabular}{| c | c | c | c |} 
\hline
 Procedure  & Empirical FDR & FDR 95\% one-sided CI  & Empirical power \\ 
\hline
  Bonfferoni & .004 & (0, .052) & 1  \\
\hline
  Benjamini-Hochberg's &  .018 & (0, .134) & 1  \\
\hline
 Hochberg's  & .016 & (0, .127) & 1 \\
\hline
 Holm's  & .013 &  (0, .114) & 1  \\
\hline
\end{tabular}
\end{center}
\end{table}


\section{Model selection and FDR controlling}
\label{sim:sec_fdr}
In this section, we implemented Bonferroni, Benjamini-Hochberg's, Hochberg's, and Holm's procedures to detect components of $\truth$ that are significantly different from 0 while controlling the false discovery rate (FDR) at level $q = 0.05$. We provide the simulated FDR and power in Table \ref{t3}. The hypotheses are $H_{0,i}: (\truth)_i = 0$ vs. $H_{1,i} : (\truth)_i \neq 0$ for $i = 1,\ldots, 6$. Simulation results suggest that all four proceudres are able to correctly detect all non-zero parameters and control the false discovery rate below the predefined threshold $q$. For smaller networks with 200 nodes or more, the four procedures have empirical power of 1 and FDR below $q$.

